Studies of highly-boosted top quarks near the TeV scale using jet masses at the LHC

Studies of highly-boosted top quarks produced inclusively in pp collisions at 14 TeV are discussed. The hadronic decays of boosted top quarks was studied in a data-driven approach by analysing shapes of jet-mass distributions. Using Monte Carlo models after a fast detector simulation, it is shown that inclusive production of boosted top quarks can be observed if it has a cross section at least twice larger than the prediction from the approximate next-to-next-to-leading-order (aNNLO) calculation for the ttbar process. The ttbar process with the nominal aNNLO strength can be measured using the masses of jets after a b-tagging.

==> definitions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% isEM variables
%
% Hadronic leackage
\newcommand{\Rhad}    {\ensuremath{R_{\rm had}}}
\newcommand{\Rhadone} {\ensuremath{R_{\rm had_{1}}}}

% Middle
\newcommand{\Reta}    {\ensuremath{R_{\eta}}}
\newcommand{\Rphi}    {\ensuremath{R_{\phi}}}
\newcommand{\wetatwo} {\ensuremath{w_{2}}}

% Strips
\newcommand{\Fside}   {\ensuremath{F_{\rm side}}}
\newcommand{\wthree}  {\ensuremath{w_{s\,3}}}
\newcommand{\wtot}    {\ensuremath{w_{s\,{\rm tot}}}}
\newcommand{\DeltaE}  {\ensuremath{\Delta{}E}}
\newcommand{\Eratio}  {\ensuremath{E_{\rm ratio}}}
\newcommand{\Emaxtwor}{\ensuremath{R_{\rm max\,1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mo}      {\ensuremath{^{-1}}}

\newcommand{\Etg}     {\ensuremath{E_{T}^{\gamma}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%for efficiency section
\newcommand{\effID}{\hbox{$\varepsilon^{{\rm offl}}$}}
\newcommand{\effReco}{\hbox{$\varepsilon^{{\rm reco}}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%for purity section
\newcommand{\EtCone}{\et^{(R<0.4)}}

\newcommand{\obs}{^\mathrm{obs}}
\newcommand{\sig}{^\mathrm{sig}}
\newcommand{\bkg}{^\mathrm{bkg}}
\newcommand{\Ns}{N\sig}
\newcommand{\Nb}{N\bkg}
\newcommand{\N}{N\obs}

\newcommand{\pdf}{\Pi}
\newcommand{\ph}{_\gamma}
\newcommand{\MC}{_\mathrm{MC}}
\newcommand{\data}{_\mathrm{data}}

\newcommand{\iso}{\mathrm{Iso}(\mu)}

\newcommand{\etaM}{|\eta_\mathrm{S2}|}


\newcommand{\ptjet}{p_{T}(\mathrm{jet})}
\newcommand{\pttop}{p_{T}(\mathrm{top})}
\newcommand{\jetpt}{p_{T}(\mathrm{jet})}

\newcommand{\etajet}{\eta(\mathrm{jet})}
\newcommand{\etatop}{\eta(\mathrm{top})}
\newcommand{\mtop}{m(\mathrm{top})}


\newcommand{\ntrk}{N(\mathrm{tracks})}
\newcommand{\mjet}{M_{\mathrm{jet}}}
\newcommand{\mcl}{M_{\mathrm{cl.pair}}}
\newcommand{\ecjet}{EC_{\mathrm{jet}}}

\newcommand{\Equation}[2]{\begin{equation} #2 \label{#1} \end{equation} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

